Denoising and Selecting Pseudo-Heatmaps for Semi-Supervised Human Pose Estimation

We propose a new semi-supervised learning design for human pose estimation that revisits the popular dual-student framework and enhances it two ways. First, we introduce a denoising scheme to generate reliable pseudo-heatmaps as targets for learning from unlabeled data. This uses multi-view augmentations and a threshold-and-refine procedure to produce a pool of pseudo-heatmaps. Second, we select the learning targets from these pseudo-heatmaps guided by the estimated cross-student uncertainty. We evaluate our proposed method on multiple evaluation setups on the COCO benchmark. Our results show that our model outperforms previous state-of-the-art semi-supervised pose estimators, especially in extreme low-data regime. For example with only 0.5K labeled images our method is capable of surpassing the best competitor by 7.22 mAP (+25% absolute improvement). We also demonstrate that our model can learn effectively from unlabeled data in the wild to further boost its generalization and performance.

==> tables/ablation_PLA_VS_Vanilla.tex <==
\begin{table}[!htbp]
\begin{center}
\resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{lll}
            \toprule
            Augmentation & Selection & mAP  \\
            \hline
            1 weak & N/A  & 42.67  \\ 
            (1 + K) weak  & avg &  42.11     \\  
            (1 + K) weak  & max &  43.74     \\
            \hline
            1 weak + K strong & avg     & 39.58  \\
            1 weak + K strong & max     & \textbf{44.91}  \\
            
            \bottomrule
    \end{tabular}
}
\end{center}
    \vskip -1.5em
    \caption{\small \it \textbf{Comparison between PLA and multi-transform ensemble.} The two key differences between PLA and multi-transform are 1) the selection scheme and 2) using auxiliary strong augmentation to produce pseudo-labels. Both differences result in key performance improvement. Results are shown without threshold-and-reconstruct and K is set to 5.}
    \label{tab:ablation_pla_vs_vanilla}
\end{table}
